Absence of long range order in the frustrated magnet SrDy$_2$O$_4$ due to trapped defects from a dimensionality crossover

Magnetic frustration and low dimensionality can prevent long range magnetic order and lead to exotic correlated ground states. SrDy$_2$O$_4$ consists of magnetic Dy$^{3+}$ ions forming magnetically frustrated zig-zag chains along the c-axis and shows no long range order to temperatures as low as $T=60$ mK. We carried out neutron scattering and AC magnetic susceptibility measurements using powder and single crystals of SrDy$_2$O$_4$. Diffuse neutron scattering indicates strong one-dimensional (1D) magnetic correlations along the chain direction that can be qualitatively accounted for by the axial next-nearest neighbour Ising (ANNNI) model with nearest-neighbor and next-nearest-neighbor exchange $J_1=0.3$ meV and $J_2=0.2$ meV, respectively. Three-dimensional (3D) correlations become important below $T^*\approx0.7$ K. At $T=60$ mK, the short range correlations are characterized by a putative propagation vector $\textbf{k}_{1/2}=(0,\frac{1}{2},\frac{1}{2})$. We argue that the absence of long range order arises from the presence of slowly decaying 1D domain walls that are trapped due to 3D correlations. This stabilizes a low-temperature phase without long range magnetic order, but with well-ordered chain segments separated by slowly-moving domain walls.

==> author_list_jan2017.tex <==
\author{N. Gauthier}  
\email{nicolas.gauthier4@gmail.com}
\affiliation{Laboratory for Scientific Developments and Novel Materials, Paul Scherrer Institut, 5232 Villigen, Switzerland}

\author{A. Fennell} 
\affiliation{Laboratory for Neutron Scattering and Imaging, Paul Scherrer Institut, 5232 Villigen, Switzerland}

\author{B. Pr\'evost}
\affiliation{D\'epartement de Physique \& Regroupement Qu\'eb\'ecois sur les Mat\'eriaux de Pointe (RQMP), Universit\'e de Montr\'eal, Montr\'eal, Qu\'ebec H3C 3J7, Canada}

\author{A.-C. Uldry}
\affiliation{Condensed Matter Theory Group, Paul Scherrer Institut, 5232 Villigen, Switzerland}

\author{B. Delley}
\affiliation{Condensed Matter Theory Group, Paul Scherrer Institut, 5232 Villigen, Switzerland}

\author{R. Sibille}
\affiliation{Laboratory for Neutron Scattering and Imaging, Paul Scherrer Institut, 5232 Villigen, Switzerland}

\author{A. D\'esilets-Benoit}
\affiliation{D\'epartement de Physique \& Regroupement Qu\'eb\'ecois sur les Mat\'eriaux de Pointe (RQMP), Universit\'e de Montr\'eal, Montr\'eal, Qu\'ebec H3C 3J7, Canada}

\author{H.A. Dabkowska} 
\affiliation{Brockhouse Institute for Materials Research, Hamilton, Ontario L8S 4L8, Canada}

\author{G. Nilsen}
\affiliation{Institut Laue-Langevin, CS 20156, F-38042 Grenoble Cedex 9, France}

\author{L.-P. Regnault}
\affiliation{Institut Laue-Langevin, CS 20156, F-38042 Grenoble Cedex 9, France}

\author{J.S. White}
\affiliation{Laboratory for Neutron Scattering and Imaging, Paul Scherrer Institut, 5232 Villigen, Switzerland}

\author{C. Niedermayer}
\affiliation{Laboratory for Neutron Scattering and Imaging, Paul Scherrer Institut, 5232 Villigen, Switzerland}

\author{V. Pomjakushin}
\affiliation{Laboratory for Neutron Scattering and Imaging, Paul Scherrer Institut, 5232 Villigen, Switzerland}

\author{A.D. Bianchi} 
\affiliation{D\'epartement de Physique \& Regroupement Qu\'eb\'ecois sur les Mat\'eriaux de Pointe (RQMP), Universit\'e de Montr\'eal, Montr\'eal, Qu\'ebec H3C 3J7, Canada}

\author{M. Kenzelmann}
\email{michel.kenzelmann@psi.ch}
\affiliation{Laboratory for Scientific Developments and Novel Materials, Paul Scherrer Institut, 5232 Villigen, Switzerland}
\vskip 0.25cm


==> supplementary170205.tex <==


\section{Calculation of the Zeeman splitting tensor}
\label{appendixGtensor}
For a doublet ground state, it is possible to write the Zeeman energy Hamiltonian in terms of an effective spin $S=\frac{1}{2}$. The original Hamiltonian is defined by
$\mathcal{H}_\text{Zeeman}=\sum_{\alpha} H_\alpha  \hat{M}_\alpha$
where the index $\alpha$ indicates the axes $x$, $y$ and $z$, $H_\alpha$ is the magnetic field and $\hat{M}_\alpha$ is the magnetization operator. The magnetization operator is defined as $\hat{\bf{M}}=\hat{\bf{L}}+2\hat{\bf{S}}$, where $\hat{\bf{L}}$ and $\hat{\bf{S}}$ are the orbital and spin operators respectively. The Hamiltonian can be rewritten for an effective spin $S=\frac{1}{2}$ as
$\mathcal{H}_\text{Zeeman}=\mu_B \sum_{\alpha \beta} H_\alpha g_{\alpha \beta} \hat{S}_\beta$
where $\hat{S}_\alpha$ is the effective spin-$\frac{1}{2}$ operator and $g_{\alpha \beta}$ forms the $\bf{g}$-tensor. Assuming that the doublet wavefunctions are $\ket{+}$ and $\ket{-}$, the elements of the $\bf{g}$-tensor can be evaluated from the matrix elements of $\hat{\bf{M}}$:
\begin{equation}
\begin{aligned}
g_{\alpha x} &= 2 \text{Re} \bra{+} \hat{M}_\alpha \ket{-}/ \mu_B, \\
g_{\alpha y} &= -2 \text{Im} \bra{+} \hat{M}_\alpha \ket{-}/ \mu_B, \\
g_{\alpha z} &= 2  \bra{+} \hat{M}_\alpha \ket{+}/ \mu_B.
\end{aligned}
\end{equation}
The $g$-factors along the principal axes are obtained from the matrix $\bf{G}=\bf{g} \cdot  \bf{g}^T$. The square-root of the eigenvalues of $\bf{G}$ are the $g$-factors along the principal axes, which are themselves defined by the eigenvectors.\cite{Weil2006,Malkin2015} 
\newline

In the presence of a mirror plane perpendicular to $z$ at the magnetic ion site, the matrix $\bf{G}$ simplifies to
\begin{equation}
\bf{G}=\begin{bmatrix}    G_{xx} &  G_{xy}   & 0 \\  G_{xy}  &  G_{yy}   & 0 \\    0 &   0. & G_{zz} \end{bmatrix}.
\end{equation}
In that case, one of the principal axis points along $z$ while the two others are in the $xy$-plane. This is the case for the magnetic ions in \sdo\ with a mirror plane perpendicular to the $c$-axis.
\newline

To evaluate the $\bf{g}$-tensor of the Dy$^{3+}$ ions in \sdo, the matrix elements of the magnetization operator $\hat{\bf{M}}$ have to be calculated for the doublet ground state. The wavefunctions obtained by the \textit{multiX} software were used for this calculation. The \textit{multiX} software \cite{Uldry2012} calculates the single-ion energy levels in the presence of crystalline electric fields. Slater determinants of the electronic configuration are used as the wavefunction basis. The matrix elements of $\hat{\bf{M}}$ have been calculated from this basis by using the Slater-Condon rules for the doublet ground state of the two inequivalent Dy$^{3+}$ sites. The $\bf{g}$-tensor, $g$-factors and principal axes were then calculated according to equations presented here. 

%\subsection{Results for Dy$^{3+}$ on site 1 for \sdo}
%\label{results1}
%The elements of the $\bf{g}$-tensor have been evaluated from the doublet ground state wavefunctions calculated by \textit{multiX} on the Dy$^{3+}$ inequivalent site 1. The resulting $\bf{G}$-matrix is:
%\begin{equation}
%\bf{G}=\begin{bmatrix}    64.72 &  1.88   & 0.00 \\  1.88  &  8.16   & 0.00 \\    0.00 &   0.00  & 70.76 \end{bmatrix}
%\end{equation}
%The eigenvalues are 64.78, 8.09 and 70.76. The square-root of these values give the principal values $g_1= 8.05$, $g_2= 2.85$ and $g_3=8.41$. The eigenvectors are:
%\begin{equation}
%\begin{bmatrix}  0.9995  \\ -0.0331  \\   0.0000   \\ \end{bmatrix},
%\begin{bmatrix}   0.0331  \\ 0.9995  \\   0.0000  \\ \end{bmatrix} \text{ and }
%\begin{bmatrix}   0.0000 \\  0.0000 \\  1.0000   \\ \end{bmatrix}.
%\end{equation}
%The arccosines of the eigenvectors indicate the angles of the principal axes relative to the $x$, $y$ and $z$ axes:
%\begin{equation}
%\begin{bmatrix}  1.8982  \\ 91.8982  \\   90.0000   \\ \end{bmatrix},
%\begin{bmatrix}   88.1018  \\ 1.8982  \\   90.0000  \\ \end{bmatrix} \text{ and }
%\begin{bmatrix}   90.0000 \\   90.0000 \\  0.0000   \\ \end{bmatrix}.
%\end{equation}
%The  $g_1$ axis is in the $ab$ plane at 1.9\degree\ from the $a$-axis, the $g_2$ axis is in the $ab$ plane at 1.9\degree\ from the $b$-axis and the $g_3$ axis is along the $c$-axis.   
%
%\subsection{Results for Dy$^{3+}$ on site 2 for \sdo}
%\label{results2}
%The elements of the $\bf{g}$-tensor have been evaluated from the doublet ground state wavefunctions calculated by \textit{multiX} on the Dy$^{3+}$ inequivalent site 2. The resulting $\bf{G}$-matrix is:
%\begin{equation}
%G=\begin{bmatrix}    13.44 &  -71.03 &   0.00 \\   -71.03 &  375.31 &    0.00 \\    0.00 &    0.00 &   0.00 \end{bmatrix}
%\end{equation}
%The eigenvalues are   388.76, 0.00 and 0.00. The square-root of these values give the principal values $g_1= 19.72$, $g_2= 0.00$ and $g_3=0.00$. The eigenvectors are:
%\begin{equation}
%\begin{bmatrix}  -0.1860   \\  0.9826  \\   0.0000 \end{bmatrix},
%\begin{bmatrix}   0.9826  \\ 0.1860  \\ 0.0000 \end{bmatrix}  \text{ and }
%\begin{bmatrix}   0.0000 \\  0.0000 \\  1.0000  \end{bmatrix}.
%\end{equation}
%The arccosines of the eigenvectors indicate the angles of the principal axes relative to the $x$, $y$ and $z$ axes:
%\begin{equation}
%\begin{bmatrix}  100.7170  \\ 10.7170  \\   90.0000   \\ \end{bmatrix},
%\begin{bmatrix}   10.7170  \\  79.2830   \\   90.0000  \\ \end{bmatrix} \text{ and }
%\begin{bmatrix}    90.0000 \\   90.0000 \\   0.000  \\ \end{bmatrix}.
%\end{equation}
%The $g_1$ axis is in the $ab$ plane at 10.7\degree\ from the $b$-axis, the $g_2$ axis is in the $ab$ plane at 10.7\degree\ from the $a$-axis and the $g_3$ axis is along the $c$-axis.         


